NatGen: Generative pre-training by "Naturalizing" source code

Pre-trained Generative Language models (e.g. PLBART, CodeT5, SPT-Code) for source code yielded strong results on several tasks in the past few years, including code generation and translation. These models have adopted varying pre-training objectives to learn statistics of code construction from very large-scale corpora in a self-supervised fashion; the success of pre-trained models largely hinges on these pre-training objectives. This paper proposes a new pre-training objective, "Naturalizing" of source code, exploiting code's bimodal, dual-channel (formal & natural channels) nature. Unlike natural language, code's bimodal, dual-channel nature allows us to generate semantically equivalent code at scale. We introduce six classes of semantic preserving transformations to introduce un-natural forms of code, and then force our model to produce more natural original programs written by developers. Learning to generate equivalent, but more natural code, at scale, over large corpora of open-source code, without explicit manual supervision, helps the model learn to both ingest & generate code. We fine-tune our model in three generative Software Engineering tasks: code generation, code translation, and code refinement with limited human-curated labeled data and achieve state-of-the-art performance rivaling CodeT5. We show that our pre-trained model is especially competitive at zero-shot and few-shot learning, and better at learning code properties (e.g., syntax, data flow).

==> body/3.method.bck.tex <==
\section{SemCode}
\label{sec:method}


In this section, we discuss the methodology of \tool. We divide \tool's approach into three steps: (i) ``De-Naturalize'' source code to accumulate pre-training data for \tool (\S\ref{sec:semantic_denoising}); (ii) pre-train \tool using this data for naturalization task (\S\ref{sec:pretrain_train}); (iii) Finetune pre-trained \tool with task specific dataset (\S\ref{sec:finetuning}). 
% In this section, we discuss the methodology for \tool. We divide \tool's approach into three parts. In first step, we ``De-Naturalize'' source code and accumulate pre-training data for \tool (\S\ref{sec:semantic_denoising}). Second, we pre-train \tool using this data for naturalization task (\S\ref{sec:pretrain_train}). And finally, we finetune pre-trained \tool with task specific dataset (\S\ref{sec:finetuning}). 

% \tool's approach is divided into two parts. First, we pre-train \tool to naturalize code; next, we fine-tune it on task. 
%that is syntactically, \emph{and} semantically correct. 

\input{figures/approach}

% \input{figures/pretrain}
\subsection{De-Naturalizing Source Code}
%\subsection{Generating pre-training data}
\label{sec:semantic_denoising}
%\rayb{Read this}

%As explained above (\S~\ref{sec:naturalizing}) 
Our pre-training approach involves generating very large volumes of code-naturalization training data. To de-naturalize code, we consider a set of semantic-preserving,  ``de-naturalizing'' code transformation patterns $\Phi = \{\phi_1, \phi_2,  \phi_3, ...\}$. 
Given a code $c_i$, $\phi_j(c_i)$ transforms the code in a way that changes the structure of the code while maintaining the semantic equivalence with the previous code. These transformations are meaning-preserving but artificially transformed code from its original (human-) written form. 
%We discuss details about these transformation patterns in \cref{sec:data_prep}.  

\Cref{fig:approach} shows the workflow of generating the pre-traininf dataset. Given a piece of source code ($c_i$), we first extract the AST ($T_{c_i}$), using a parser. We use tree-sitter\footnote{\url{https://tree-sitter.github.io/tree-sitter/}} to parse the source code. For the AST, we extract potential locations for de-naturalization. These locations are nodes ($n_k$) in $T_{c_i}$. While choosing location $n_k$ from $T_{c_i}$, we consult $\Phi$ -- we extract the nodes where at least one of $\phi_j \in \Phi$ is applicable. Once we have a set of such nodes, we filter out the transformation rules that cannot be applied to any node of in $T_{c_i}$. After such a filtration, we have a set of transformations $\Phi_a \subseteq \Phi$. At this stage, we randomly select one transformation pattern $\phi_j \in \Phi_a$ to apply at an application location (AST node) $n_k$.  We apply $\phi_j$ to $n_k$ to get the transformed node $n'_{k}$. We then structurally match $n'_{k}$ with the original AST $T_{c_i}$, specifically $n_k$. We adapt the context of $n_k$ to the transformed node's ($n'_k$) context. In that way, we get the transformed AST ($T'_{c_i}$) -- which we then translate to get the transformed code $c'_i$. We designed the transformation function $\phi_j$ and subsequent context adaptation in such a way that preserves the meaning or functionality of the original code. We use AST analysis and (approximated) data flow analysis on code AST. 

% As explained above (\S~\ref{sec:naturalizing}) our pre-training approach involves generating very large volumes of code-naturalization training data. For 
% this, we apply meaning-preserving, ``de-naturalizing" transformations
% to naturally-occurring code in mature Open-source projects. These transformations are meaning-preserving, but artificially
% transform code from their originally (human-) written form. Now, the original code is paired with this de-naturalized code. The pre-training
% task is to learn to rewrite the de-naturalized code into it's original, ``natural" form.  In the sections following, we describe the de-naturalizing transforms that we use. 


%\subsection{Semantic Noise Inducing Transformation}
\paragraph{\textbf{``De-naturalizing'' Transformations.}}
\label{sec:data_prep}
\input{body/example_code/transformations}
In this section, we describe semantic-preserving, de-naturalizing transformation functions. Casalnuovo \emph{et al}~\cite{casalnuovo2020programmers,casalnuovo2020does} showed that transforming code from what developers' had written to other forms generally makes it less natural (higher in cross-entropy according to language models) and also reduces human comprehension speed, and comprehension accuracy. 
Nevertheless, we use six classes of such semantics-preserving, 
de-naturalizing transformations. 
% to introduce ``unnaturalness'' semantic noises into the training data. 
These transformations are motivated by prior work on functional reasoning about source code~\cite{ding2021contrastive, gopstein2018prevalence, gopstein2020thinking} and semantic bug-seeding~\cite{patra2021semantic}. 
% We remind the user that 
% Earlier work by 


\subsubsection{{Loop Transformation.}}
\label{sec:loop_transformation}
This transformation modifies {\tt for} loops into equivalent {\tt while} loop and vice-versa. We rewrite a {\tt while} loop of the form~\texttt{ while ( \highlight{condition} )}~\texttt{\{ loop-body \}} into a {\tt for} loop as ~\texttt{ for ( \highlight{\textbf{;}} \highlight{condition} \highlight{\textbf{;}} )}~\texttt{\{ loop-body \}}. \Cref{fig:loop_transformation} shows one such example. Likewise, to transform a {\tt for} loop into a {\tt while} loop, we move the initializer of the {\tt for} (if any) before the loop, and the update {\em expression} (if any) of the {\tt for} loop as the last {\em statement} in the loop. We also add this update statement before any loop breaking statement (\ie \texttt{break}, \texttt{continue}). For example, we transform ``\texttt{for(\highlight{int i = 0;} i < 10; \highlight{i++})\{ if(i)\{ foo(); continue;\}  bar(); \}}'' as ``\texttt{\highlight{int i = 0;} while(i < 10)\{ if(i)\{ foo(); \highlight{i++;} continue;\}  bar(); \highlight{i++;}\}}''.

\subsubsection{{Dead Code Injection.}}
\label{sec:dead_code}
We inject blocks of dead code at random positions in the original code. 
%\prem{Check this!} 
By ``dead code" we mean code that appears in the source but is
never executed.
For instance, \Cref{fig:dead_code} shows an example of dead code injection. Here we inject the code block \linecode{if( arr [mid] < key)\{ ...\}} at line 4 of the original code (\cref{fig:original_code}). To add challenge to the model, we transplant these inserted statements from the same input code. To ensure the "death" of inserted code, we put the inserted statements in a block headed by either a loop or a branch,
where  the condition of the loop or the branch can never be satisfied \ie the code inside the block will never execute. In \Cref{fig:dead_code}, the condition \highlight{\tt i < i} is always \linecode{false}; and the code in line 5 is quite dead.

\subsubsection{{Block Swap.}}
\label{sec:block_swap}
In this transformation, we swap the ``then" block of a chosen {\tt if} statement with the corresponding {\tt else} block.  To preserve semantic equivalence, we negate the original branching condition. For instance, \cref{fig:block_swap} replaces the {\tt if} block (line 4 in \Cref{fig:original_code}) with the {\tt else} block (line 5 in \cref{fig:original_code}). We negate the original condition (\linecode{arr[mid] == key}) as (\linecode{arr[mid] != key}).


\subsubsection{{Operand Swap.}}
\label{sec:operand_swap}
Here, we swap the operands of binary (i) logical operations, and (ii) arithmetical operation (only addition and multiplication). For instance, we change the statement \linecode{high = mid + 1} with \linecode{high = 1 + mid} in line 6 in \Cref{fig:block_swap}. In case of logical operator, when swapping the operands, we also make sure the modified expression is the logical equivalent to the one before modification. For examples, when we rewrite \linecode{foo >= bar}, we rewrite as \linecode{bar <= foo}.
% \prem{Example of logical op swap?}

\subsubsection{{Confusing Code Insertion.}}
\label{sec:confusion_removal}
We introduce confusing code patterns in the code as outlined by \citet{gopstein2018prevalence, gopstein2020thinking}. In particular, we introduce two forms of confusing code. First, we modify the of the form \linecode{\{i = j; j += 1;\}} to \linecode{i = j++;}. Second, we introduce ternary operator wherever applicable. For example, we transform the code \linecode{if (x != 0) \{y = p;\} else \{y = q;\}} to \linecode{y = (x != 0) ? p : q;}. 

\subsubsection{{Variable Renaming.}}
\label{sec:var_renaming}
We transform code by renaming some variables to {\tt VAR\_i}. While renaming a variable, we analyze the dataflow of that variable and rename all occurrences of that variable in the entire code. From all the variables used in the code, we change jsut a certain percentage. For instance, in \Cref{fig:var_renaming}, we renamed variable \linecode{arr} to \linecode{var_1}, and variable \linecode{high} to \linecode{var_2}, leaving all other variables unchanged. Note that, unlike other transformations, variable renaming does not create AST of Dataflow graph difference. However, this challenging task~\cite{allamanis2017learning} forces the model to learn to generate natural variable names.



\subsection{Pre-training}
\label{sec:pretrain_train}
Given an developer written code $c_i$, we first make it ``unnatural" using one of the randomly chosen transformation from the applicable transformations as described in \Cref{sec:data_prep}. Formally, we create ``unnatural'' code using a transformation $\phi_j$ as $\phi_j(c_i)$. We then use a neural sequence-to-sequence translation model ($\mathcal{M}$) to reconstruct $c_i$ from from $\phi(c_i)$, that is, we want $\mathcal{M}(\phi_j(c_i))$ to approximate $c_i$ . In particular, given a training dataset $\mathcal{D}_t = \{c_1, c_2, ...\}$ consisting of developers written code, set of "de-naturalizing" transformations $\Phi = \{\phi_1, \phi_2, \phi_3, ...\}$, we optimize the following function to learn $\mathcal{M}$'s optimal parameter $\Theta$.

\begin{equation}
    \Theta = \argmin_{\theta} \sum_{c_i\in \mathcal{D}_t} CrossEntropy\left(\mathcal{M}\left(\phi_j\left(c_i\right)\right), c_i\right)
\end{equation}

\subsection{Finetuning}
\label{sec:finetuning}
The objective of our pre-training is to learn to both comprehend and generate general-purpose source code. However, different tasks related to source code generation (\eg text to code generation, code to code translation, bug fixing) call for task specific training of the pre-trained model to cater to the need of that task. This training phase on a pre-trained model is known as fine-tuning~\cite{devlin2018bert}. We consider the fine-tuning in \tool as a translation task, we follow the standard procedure for transformer based-machine translation~\cite{vaswani2017attention}. First, the encoder generates the encoded representation $R(X)$ given the input $X= [x_1, x_2, ..., x_n]$. The decoder then sequentially generates the output $Y = [y_1, y_2, ..., y_m]$. While encoding an input token $x_k$, the encoder learn the attention matrix \wrt every token in the input, including $x_k$ itself. Such attention matrix is known as {\em self-attention}. While generating an output token $y_m$, the decoder learn the attention matrix with all previsouly generated tokens $[y_1, y_2, ..., y_{m-1}]$ through {\em self-attention} and the encoder generated representation $R(X)$ through {\em cross-attention}. We refer to \citet{vaswani2017attention} for more detail about transformer based translation.


==> body/8.threats.tex <==
\section{Threats to Validity}
\label{sec:threats}

\paragraph{Internal Validity.} 
In \Cref{sec:semantic_denoising}, we choose one of six transformation patterns to ``de-naturalize" source code. Thus, the model learns to ``naturalize" one transformation at a time. In fact, we observed examples, where we give the model with more than one `un-natural' code-patterns, and model reverses only one pattern. There is a threat that these patterns create biases towards learning to write ``natural'' code, since all natural code are not bound by these simple patterns. Regardless, we consider \tool as a proof-of-concept and the first work towards teaching a model to write natural code. We leave the investigation more natural code patterns and their effect on code generation as a potential future work.

\paragraph{Construct Validity.}
We initialize \tool with pre-trained checkpoint from CodeT5 (already pre-trained 75K steps with their objective) and train \tool for 25K steps with `natural-code' writing objective. A skeptic reader would want to know what happens when we pre-train CodeT5 for 25K more steps with their training objective. We argue that since the pre-training objective does not explicitly account for generating code (we refer readers to section 3.2 of CodeT5's original paper), any further training with the CodeT5 objective does not necessarily increase its code generation capacity. We do acknowledge CodeT5's ability to understand and reason about {\em input}. Since the pre-training large model is extremely expensive~(\S\ref{sec:experiemnts}), we leverage such knowledge by initializing \tool from CodeT5's publicly available pre-trained model. Moreover, CodeT5 did not release their code for pre-training, nor any earlier or later checkpoints for us to carry out further investigation. 


\subsection{External Threat.}


==> body/introduction_backup.tex <==
\section{Introduction}
\label{sec:intro}
Statistical models that capture the ``naturalness" of code~\cite{hindle2012naturalness} have proven to be quite valuable in a variety of tasks~\cite{allamanis2018survey}, including  code repair, code summarization, code retrieval,
and code clone detection. The earlier work in this area used models directly trained  on tasks, including the early work on  type recovery~\cite{hellendoorn2017deep}, de-obfuscation~\cite{raychev2014code,vasilescu2017recovering}, code repair~\cite{gupta2017deepfix, chakraborty2020codit}, and code summarization~\cite{iyer2016summarizing, ahmad2020summarization}.
 Training on-task requires a large amount of labeled data, so that the enormous number of parameters that come with modern neural models can be deployed  and configured effectively for maximum performance. 
 While labeled data is abundant for tasks like code completion (where the corpus inherently provides supervision), other tasks like summarization, code repair, etc. require careful curating to ensure that
 the data is of high quality. Simply grabbing data from Github might lead to poor quality~\cite{gros2020code}, and high levels of duplication~\cite{allamanis2019adverse}. 
 As model capacity has increased (capacities in the range of tens of  billions of parameters are now routine) this unacceptable disparity between vast model capacity and the limited availability of well-curated, high-quality, labeled data has increased, and will likely  grow worse. 
 
This shortage, of high-quality labeled data for on-task training is not a problem peculiar to software engineering (although it is more acute here, since the required manual labeling effort might demand a much higher level of specialized skill than with natural language tasks). 
In NLP research, the strategy currently in vogue for dealing with this problem involve various offshoots of BERT~\cite{devlin2018bert}. The key insight here is that independent of final tasks, when \emph{very} high capacity models are trained, over enormous data sets, on simple, self-supervised, ``busy work'' tasks,  they  still \emph{learn representations that are useful on \underline{actual} tasks}. Furthermore, these cheaply-learned representations can then be used to train highly performant models \emph{even} with relatively small amounts of high-quality on-task training data. These two steps, known as ``pre-training" and ``fine-tuning" now yield SOTA performance on a wide range of tasks. 
 
 
For Natural Language, the ``busy work'' pre-training tasks include such tasks as:  guessing masked words in context; guessing the next sentence in context; and de-noising a given, corrupted sentence. Using harder pre-training tasks appears to 
  %force the learned representations to capture more useful structural and semantic properties of text, and 
  lead to better fine-tuned on-task performance. This is achieved in two different ways: first, using harder pre-training tasks forces models to 1) learn \emph{better internal representations of
  the given inputs} ({\eg} being forced to fill in several blanks forces
  the model to learn better statistics of text patterns); 2) making the generation part of pre-training harder (\emph{e.g.,} T5 forces a complex generation task, and NXP in BERT forces next sentence generation) forces the models to become \emph{better at the generation of sequential text}. 
  
 We propose a novel kind of ``busy work" task that places stronger demands during pre-training. Our idea is inspired by noting
  the kind of work that human Editors
  (of books, journals, newspapers) perform: they digest imperfectly written, but mostly correct text, understand the intent, and then produce more perfect text, with pretty-much the same meaning. Editing is \underline{\emph{hard}}: a skilled Editor has to have very high levels of language comprehension, to understand given, potentially badly-written text, \emph{and then} deploy very high-level writing
  skills to generate well-formed text. 
  If Editing could be used as an at-scale pre-training task, the learned model would presumably have very good language comprehension, and also generate excellent text. But it's not at all obvious how to generate at-scale training data   for this ``Editing" task, say, for English. 
  
  But our concern here is code, not natural language. We start with the argument that, because of 
  bimodal, dual-channel nature of code~\cite{casalnuovo2020theory}, it is indeed possible to generate at-scale training data for the Editing task.
  Code has a formal channel, with well-defined semantics; because of this,
  it's possible to transform code into different forms, while 
  \emph{preserving meaning}. Essentially, we can deploy a set of meaning preserving transformations to \emph{rewrite} existing code from widely-used
  github projects (which presumably have good-quality code that has passed human code review). These rewrites preserve meaning, but will make the code into an artificial, often unnatural form\footnote{Studies, with human-subjects~\cite{casalnuovo2020does,casalnuovo2020programmers} show that humans find such rewritten but semantically identical forms harder to read and
  understand.}. We now have a matched pair, of two semantically forms of code: an ``unnatural" form, and the original form; furthermore we can produce these pairs, at scale. Using large numbers of such pairs, we can pre-train on a challenging code ``Naturalization" task, which then, by analogy with human Editors as described above, forces the pre-trained model to learn to do two hard things: 1) first, capture the meaning of the input code, and 2) generate an output that more closely resembles the code that human coders write. Our hypothesis that the resulting model will both learn better meaning representations, \emph{and also} generate better code. 
  
  We can now summarize our main contributions
  
  \begin{enumerate}
      \item We introduce the idea of "Code naturalization" as a pre-training task. 
     \item Using code from Github, and custom tooling, we have generated (and will release) a large dataset for pre-training models on the Naturalization task. 
     \item We have built (and will release) a large CodeT5~\cite{wang2021codet5} model pre-trained on Naturalization. 
     \item We show that (when appropriately fine-tuned) this \tool outperforms SOTA on several tasks. 
  \end{enumerate}

% All our models, tools, and data will be released whenever this paper is finally published. 
We publish our source code and data download sript for pretraining \tool anonymously in  \url{https://github.com/natgen-team/NatGen}. We also share all the trained models in \url{https://drive.google.com}.

\medskip
 
%  \noindent\saikat{This is Saikat's}

% \noindent\toufiq{This is Toufiq's}

% \noindent\robin{This is Robin's}

% \noindent\rayb{This is Baishakhi's}

% \noindent\prem{This is Prem's}

% \cite{CodeXGLUE}

==> figures/pretrain.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/pretrain.pdf}
    \caption{Pre-training by ``Naturalizing'' source code.}
    \label{fig:pretraining_enc_dev}
\end{figure}

==> figures/rq1/training_performance.tex <==
% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=.75\linewidth]{images/rq1/training_accuracy_over_steps.pdf}
%     \caption{Progression of different metrics on evaluation dataset over training time.}
%     \label{fig:pretrain_progression}
% \end{figure}



==> figures/rq1/transformation_count_stat.tex <==
% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=\linewidth]{images/rq1/Transformation_count_statistics.pdf}
%     \vspace{-0.3cm}
%     \caption{Statistics of Rewriting rules.}
%     \label{fig:transfromation_count_stat}
% \end{figure}

==> tables/statistical_result.tex <==
\begin{table}[!htb]
    \centering
    \small
    \caption{One sided Wilcoxon sign rank test statistics result comparison between \tool and CodeT5 across different tasks and metrics. \colorbox{highlight}{Highlighted} results are statistically significant with $>$95\% confidence.}
    \begin{tabular}{llr}
        \hlineB{2}
        Task & Metric & P-Value \bigstrut\\
        \hlineB{2}
        \multirow{2}{*}{Code generation} & Syntax Match   &  \colorbox{highlight}{$<$0.001} \bigstrut[t]\\
                                         & Dataflow Match &  \colorbox{highlight}{$<$0.001} \\
        \multirow{-2}{*}{(Text to Java)} & CodeBLEU       &  \colorbox{highlight}{$<$0.001} \bigstrut[b]\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \hlineB{2}
        \multirow{2}{*}{Translation}     & Syntax Match   &  0.093 \bigstrut[t]\\
                                         & Dataflow Match &  0.147 \\
        \multirow{-2}{*}{(C\# to Java)}  & CodeBLEU       &  \colorbox{highlight}{0.016} \bigstrut[b]\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \hlineB{2}
        \multirow{2}{*}{Translation}     & Syntax Match   & 0.166 \bigstrut[t]\\
                                         & Dataflow Match &  0.462 \\
        \multirow{-2}{*}{(Java to C\#)}  & CodeBLEU       &  \colorbox{highlight}{0.021} \bigstrut[b]\\
        \hlineB{2}
    \end{tabular}
    \label{tab:stat_table}
\end{table}
